Linking Scientific Instruments and HPC: Patterns, Technologies, Experiences

Powerful detectors at modern experimental facilities routinely collect data at multiple GB/s. Online analysis methods are needed to enable the collection of only interesting subsets of such massive data streams, such as by explicitly discarding some data elements or by directing instruments to relevant areas of experimental space. Such online analyses require methods for configuring and running high-performance distributed computing pipelines--what we call flows--linking instruments, HPC (e.g., for analysis, simulation, AI model training), edge computing (for analysis), data stores, metadata catalogs, and high-speed networks. In this article, we review common patterns associated with such flows and describe methods for instantiating those patterns. We also present experiences with the application of these methods to the processing of data from five different scientific instruments, each of which engages HPC resources for data inversion, machine learning model training, or other purposes. We also discuss implications of these new methods for operators and users of scientific facilities.

==> Figs/flows/flow_defs.tex <==



\section{SSX:}
From production flow:
https://github.com/globus-gladier/gladier-kanzus/tree/main/gladier_kanzus/flows

\subsection{Data Transfer flow:}
https://github.com/globus-gladier/gladier-kanzus/blob/main/gladier_kanzus/flows/flow_data_transfer.py

\begin{enumerate}
\item TRANSFER >> 'gladier_kanzus.tools.TransferOut'
\end{enumerate}

\subsection{DIALS stills flow:}
https://github.com/globus-gladier/gladier-kanzus/blob/main/gladier_kanzus/flows/flow_stills.py

\begin{enumerate}
\item         TRANSFER >> 'gladier_kanzus.tools.TransferOut',
\item         FUNCX >> 'gladier_kanzus.tools.WaitTrigger',
\item         FUNCX >> 'gladier_kanzus.tools.CreatePhil',
\item         FUNCX >> 'gladier_kanzus.tools.DialsStills',
\item         FUNCX >> 'gladier_kanzus.tools.SSXGatherData',
\item         FUNCX >> 'gladier_kanzus.tools.SSXPlot',
\item         FUNCX >> 'gladier_tools.publish.gatherMetadata',
\item        TRANSFER >>  'gladier_tools.publish.transferMetadata',
\item        INGEST >>  'gladier_tools.publish.IngestMetadata',
\item        TRANSFER >>  'gladier_kanzus.tools.TransferProc'
\end{enumerate}

\subsection{DIALS Prime flow:}
https://github.com/globus-gladier/gladier-kanzus/blob/main/gladier_kanzus/flows/flow_prime.py

\begin{enumerate}
\item FUNCX >> 'gladier_kanzus.tools.DialsPrime',
\item TRANSFER >> 'gladier_kanzus.tools.TransferPrime',
\end{enumerate}

\subsection{Data publish flow:}
https://github.com/globus-gladier/gladier-kanzus/blob/main/gladier_kanzus/flows/flow_publish.py

\begin{enumerate}
\item         FUNCX >> 'gladier_kanzus.tools.SSXGatherData',
\item         FUNCX >>  'gladier_tools.posix.tar.Tar',
\item         FUNCX >> 'gladier_kanzus.tools.SSXPlot',
\item         FUNCX >> 'gladier_kanzus.tools.DialsPlotHist',
\item        TRANSFER >>  'gladier_tools.publish.transferMetadata',
\item        INGEST >>  'gladier_tools.publish.IngestMetadata',
\item        TRANSFER >>  'gladier_kanzus.tools.TransferProc'
\end{enumerate}



\section{XPCS:}
From suresh prod repo:
https://github.com/globus-gladier/gladier-xpcs/blob/main/gladier_xpcs/flows/flow_boost.py

\subsection{XPCS online flow:}

\begin{enumerate}
\item TRANSFER >>  'gladier_xpcs.tools.TransferFromClutchToTheta',
\item FUNCX >> 'gladier_xpcs.tools.PrePublish.gatherMetadata',
\item TRANSFER >>  'gladier_xpcs.tools.PrePublish.transferMetadata',
\item INGEST >> 'gladier_xpcs.tools.PrePublish.ingestMetadata',
\item FUNCX >> 'gladier_xpcs.tools.AcquireNodes',
\item FUNCX >> 'gladier_xpcs.tools.BoostCorr',
\item FUNCX >> 'gladier_xpcs.tools.MakeCorrPlots',
\item FUNCX >> 'gladier_xpcs.tools.gather_xpcs_metadata.GatherXPCSMetadata',
\item FUNCX >> 'gladier_xpcs.tools.Publish.gatherMetadata', (this is different than the above)
\item 'gladier_xpcs.tools.Publish.transferMetadata',
\item 'gladier_xpcs.tools.Publish.ingestMetadata',
\end{enumerate}


\section{HEDM:}
From hemant repo:
https://github.com/globus-gladier/gladier-hedm/blob/main/gladier_hedm/flows/ff_flow.py

\subsection{FarField processing flow:}
\begin{enumerate}
\item TRANSFER >>  'gladier_hedm.tools.transfer_inject.Inject',
\item FUNCX >> 'gladier_hedm.tools.remote_prepare.RemotePrepare',
\item FUNCX >> 'gladier_hedm.tools.remote_peaksearch.RemotePeaksearch',   #### Multi - node
\item FUNCX >> 'gladier_hedm.tools.remote_transforms.RemoteTransforms',
\item FUNCX >> 'gladier_hedm.tools.remote_indexrefine.RemoteIndexrefine', #### Multi - node
\item FUNCX >> 'gladier_hedm.tools.remote_process.RemoteFindGrains',
\item FUNCX >> 'gladier_hedm.tools.transfer_extract.Extract',
\item FUNCX >> 'gladier_hedm.tools.remote_publish.gatherMetadata'
\item TRANSFER >> 'gladier_hedm.tools.remote_publish.transferMetadata'
\item INGEST >> 'gladier_hedm.tools.remote_publish.ingestMetadata'
\end{enumerate}


\section{BraggNN:}
From Zhengchun conversation:
https://github.com/AISDC/DNNTrainerFlow/blob/main/DNNTFlow.py

\begin{enumerate}
\item TRANSFER
\item FUNCX
\item TRANSFER
\end{enumerate}


\section{PTYCHO:}
From tekin repo: (new version!!!)
https://github.com/tekinbicer/apwf/blob/master/src/apwf/flows/automate_helper.py
That description is right but not well established. I only have ptycho reconstruction steps (1-3), which is 2d reconstruction. I don’t have step 4 currently (3d reconstruction) but it is useful/needed for 3d ptycho and I can definitely add. The step 5 is not clear since there is no fixed quality metrics. The publishing the data, step 6, is not something I worked on so far, and may need talking with Junjing etal (i can check if/what they might want to publish.) Step 7 can be the result of 3d recon.
Overall steps 5 and 6 do not exist now, and need clarification. I can add 4 and 7.

\begin{enumerate}
\item       TRANSFER >> "Initial transfer"
\item     TRANSFER >> "Pos Transfer"
\item  FUNCX >> Analyze
\item TRANSFER >> "Return transfer" 
\end{enumerate}

